Deep Function Machines: Generalized Neural Networks for Topological Layer Expression

In this paper we propose a generalization of deep neural networks called deep function machines (DFMs). DFMs act on vector spaces of arbitrary (possibly infinite) dimension and we show that a family of DFMs are invariant to the dimension of input data; that is, the parameterization of the model does not directly hinge on the quality of the input (eg. high resolution images). Using this generalization we provide a new theory of universal approximation of bounded non-linear operators between function spaces. We then suggest that DFMs provide an expressive framework for designing new neural network layer types with topological considerations in mind. Finally, we introduce a novel architecture, RippLeNet, for resolution invariant computer vision, which empirically achieves state of the art invariance.

==> sections/impl.tex <==
%!TEX root = ../main.tex

    \section{Implementation with Seperable Weight Kernels}
    With these theoretical guarantees given for DFMs, the implementation of the feedforward and error backpropagation algorithms in this context is an essential next step. We will consider operator neural networks with polynomial kernels. As aforementioned, in the case where a DFM has nodes with non-seperable kernels, we cannot give the guarntees we do in the following section. Therefore, a standard auto-differentiation set-up will suffice for DFMs with for example wave layers.

    Feedforward propagation is straight forward, and relies on memoizing operators
    by using the separability of weight polynomials. Essentially, integration need only
    occur once to yield coefficients on power functions. See Algorithm 1.


    For error backpropagation, we chose the most direct analogue for the loss function, in particular since we showed universal approximation using the $C^\infty$ norm, the integral norm will converge. 
\begin{definition}
    For a operator neural network $\scripto$ and a dataset $\left\{(\gamma_n(j), \delta_n(j))\right\}$ we say that the error for a given $n$ is defined by
    \begin{equation} \label{eq:error}
        E = \frac12 \int_{E_{L}}\left(\scripto(\gamma_n) - \delta_n \right)^2\;dj_L
    \end{equation}
\end{definition}
Using this definition we take gradient with respect to the coefficients of the polynomials on each weight surface. Eventially we get a recurrence relation in the same way one might for discrete neaural networks.
\begin{equation} \label{eq:rotBrelation}
  \begin{aligned}
    \rotB_{L,t} &= \int_{E_{L}}  \sum_b^{Z^{L-1}_Y} k^{L-1}_{t,b} j_L^b 
      \left[\scripto(\gamma) - \delta\right] \Psi^{L}\;dj_L. \\
    \rotB_{s,t} &= \int_{E_{(s)}}\sum_b^{Z^{(s-1)}_Y} \sum_a^{Z^{(s)}_X} 
      k^{(s-1)}_{t,b} j_s^{a+b} \Psi^{(s)} \rotB_{s+1,a}\; dj_s. \\
    \rotB_{\ell} &= \int_{E_{\ell}} \sum_a^{Z^{\ell}_X}
      j^{a+y}_{\ell} \Psi^{\ell} \rotB_{l+2, a}\; dj_{\ell}. \\
     \frac{\partial E}{\partial k^{\ell}_{x,y}} = \rotB_{l} &= \int_{E_{\ell}}
      j_{\ell}^x y^{\ell} \rotB_{\ell}\; dj_\ell.
  \end{aligned}
  \end{equation}
  where $\Psi$ is defined as $g'(T[y]+\beta).$ Using this recurrence relation, we can drastically reduce the time to update each weight by memoizing. That philosophy yields algorithm 2, and therefore we have completed the practical analohgues to these algorithms.


% Subsection: Fast forward Propagation
\subsubsection{Feed-Forward Propagation}

We will say that a function $f: \mathbb{R}^2 \to \mathbb{R}$ is numerically integrable if it can be seperated into $f(x,y) = g(x)h(y)$.

\begin{theorem}
If $\scripto$ is a operator neural network with $L$ consecutive layers, then given any $\ell$ such that $0\leq \ell <  L$, $y^{\ell}$ is numerically integrable, and if $\xi$ is any continuous and Riemann integrable input function, then $\scripto[\xi]$ is numerically integrable.
\end{theorem}

\begin{proof}
Consider the first layer. We can write the sigmoidal output of the $(\ell)^{\mathrm{th}}$ layer as a function of the previous layer; that is,
\begin{equation}
y^{\ell} = g\left(\int_{E_{\ell}} w^{\ell}(j_\ell, j_{\ell})y^{\ell}(j_{l})\; dj_{l}\right).
\end{equation}
Clearly this composition can be expanded using the polynomial definition of the weight surface. Hence
\begin {equation}
\begin{aligned}
y^{\ell} &= g\left(\int_{E_{\ell}}y^{\ell}(j_\ell)\sum_{x_{2\ell}}^{Z^{\ell}_Y}\sum_{x_{2l}}^{Z^{\ell}_X}{k_{x_{2l},x_{2\ell}}j_\ell^{x_{2l}}j_{\ell}^{x_{2\ell}}\;dj_\ell}\right) \\
&= g\left(\sum_{x_{2\ell}}^{Z^{\ell}_Y}j^{x_{2\ell}}\sum_{x_{2l}}^{Z^{\ell}_X}{k_{x_{2l},x_{2\ell}}}\int_{E_{\ell}} y^{\ell}(j_\ell)j_\ell^{x_{2l}}\; dj_\ell\right),
\end{aligned}
\end{equation}
and therefore $y^{\ell}$ is numerically integrable. For the purpose of constructing an algorithm, let $I^{\ell}_{x_{2\ell}}$ be the evaluation of the integral in the above definition for any given $x_{2\ell}$

It is important to note that the previous proof requires that $y^{\ell}$ be Riemann integrable. Hence, with $\xi$ satisfying those conditions it follows that every $y^{\ell}$ is integrable inductively. That is, because $y^{0}$ is integrable it follows that by the numerical integrability of all $l$, $\scripto[\xi] = y^{L}$ is numerically integrable. This completes the proof.
\end{proof}
Using the logic of the previous proof, it follows that the development of some inductive algorithm is possible. 


\begin{algorithm}[tb]
   \caption{Feedforward Propagation on $\scriptf$}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} input function $\xi$
   \FOR{$l \in \{0,\dots,L-1\}$}
   \FOR{$t \in Z_X^{\ell}$}
   \STATE Calculate $I^{\ell}_t = \int_{E_{\ell}} y^{\ell}(j_\ell)j_\ell^{t}\;dj_\ell.$
   \ENDFOR
   \FOR{$s \in  Z_Y^{\ell}$}
   \STATE Calculate $C^{\ell}_{s} = \sum_{a}^{Z^{\ell}_X} k_{a,s} I^{\ell}_{a}.$
   \ENDFOR
   \STATE Memoize $y^{\ell}(j)=g\left(\sum_{b}^{Z^{\ell}_Y} j^{b} C^{\ell}_{b}\right).$
   \ENDFOR
   \STATE The output is given by $\scripto[\xi] = y^{L}$.
\end{algorithmic}
\end{algorithm}






% Subsection: Fast error backpropr
\subsubsection{Continuous Error Backpropagation}
 the feed-forward of neural network algorithms is the notion of training. As is common with many non-convex problems with discretized neural networks, a stochastic gradient descent method will be developed using a continuous analogue to error backpropagation. 

As is typical in optimization, a loss function is defined as follows. 
\begin{definition}
    For a operator neural network $\scripto$ and a dataset $\left\{(\gamma_n(j), \delta_n(j))\right\}$ we say that the error for a given $n$ is defined by
    \begin{equation} \label{eq:error}
        E = \frac12 \int_{E_{L}}\left(\scripto(\gamma_n) - \delta_n \right)^2\;dj_L
    \end{equation}
\end{definition}
This error definition follows from $\mathcal{N}$ as the typical error function for $\mathcal{N}$ is just the square norm of the difference of the desired and predicted output vectors. In this case we use the $L^2$ norm on $C(E_{L})$ in the same fashion.

We first propose the following lemma as to aid in our derivation of a computationally suitable error backpropagation algorithm.


\begin{lemma}
Given some layer, $l>0$, in $\scripto$, functions of the form $\Psi^{\ell} =g'\left(\Sigma_ly^{\ell}\right)$ are numerically integrable. 
\end{lemma}

\begin{proof}
If\begin{equation}\Psi^{\ell}=g'\left(\int_{E_{(\ell -1)}}{y^{(\ell -1)} w^{(\ell -1)}\ dj_{\ell}}\right)\end{equation}
then
\begin{equation}
\Psi^{\ell}=
 g'\left(
   \sum_b^{Z^{(\ell -1)}_Y} j_{l}^{b}
   \sum_{a}^{Z^{(\ell -1)}_X} k_{a,b}^{(\ell -1)}
    \int_{E_{(\ell -1)}}{y^{(\ell -1)} j_{\ell}^a \ dj_{l-2}}
  \right)
\end{equation}
hence $\Psi$ can be numerically integrated and thereby evaluated.
\end{proof}

The ability to simplify the derivative of the output of each layer greatly reduces the computational time of the error backpropagation. It becomes a function defined on the interval of integration of the next iterated integral.

\begin{theorem}
The gradient, $\nabla E(\gamma,\delta)$, for the error function \eqref{eq:error} on some $\scripto$ can be evaluated numerically.
\end{theorem}

\begin{proof}
  Recall that $E$ over $\scripto$ is composed of $k^{\ell}_{x,y}$ for $x \in Z^{\ell}_X, y \in Z^{\ell}_Y$, and $0\leq l \leq L$.
  If we show that $\frac{\partial E}{\partial k^{\ell}_{x,y}}$ can be numerically evaluated for arbitrary, $l,x,y$, then every component of $\nabla E$ is numerically evaluable and hence $\nabla E$ can be numerically evaluated.
  Given some arbitrary $l$ in $\scripto$, let $n = \ell$.
  We will examine the particular partial derivative for the case that $n = 1$, and then for arbitrary $n$, induct over each iterated integral.

  Consider the following expansion for $n = 1$,
  \begin{align}
  \frac{\partial E}{\partial k^{L-n}_{x,y}} &= 
    \frac{\partial}{\partial k^{L-1}_{x,y}} 
    \frac{1}{2} \int_{E_{\ell}} \left[\scripto(\gamma) - \delta\right]^2\ dj_L \nonumber \\
  &= \int_{E_{\ell}} \left[\scripto(\gamma) - \delta\right] \Psi^{L} 
    \int_{E_{(\ell -1)}} j_{L-1}^x j_{L}^y y^{L-1} dj_{L-1}\ dj_L \nonumber \\
  &= \int_{E_{\ell}} \left[\scripto(\gamma) - \delta\right] \Psi^{L} j_{L}^y 
    \int_{E_{(\ell -1)}} j_{L-1}^x y^{L-1} dj_{L-1}\ dj_L \label{eq:n1case}
  \end{align}
  Since the second integral in \eqref{eq:n1case} is exactly $I^{L-1}_x$ from    \eqref{eq:ICache}, it follows that 
  
  \begin{equation}
  \frac{\partial E}{\partial k^{(n)}_{x,y}} = I^{L-1}_x
    \int_{E_{\ell}} \left[\scripto(\gamma) - \delta\right] \Psi^{L} j_{L}^y  \ dj_L
  \end{equation}
  and clearly for the case of $n=1$, the theorem holds. 

  Now we will show that this is all the case for larger $n$. 
  It will become clear why we have chosen to include $n=1$ in the proof upon expansion of the pratial derivative in these higher order cases.

  Let us expand the gradient for $n\in \{2,\dots,L\}$.
  \begin{equation} \label{eq:gradNGen}
  \begin{aligned} 
  \frac{\partial  E}{\partial k^{L-n}_{x,y}} = 
  \int_{E_{L}}  &[\scripto(\gamma)-\delta] \Psi^{L} 
   \underbrace{\int_{E_{L-1}} w^{L-1} \Psi^{L-1} 
  \idotsint_{E_{L-n+1)}} w^{L-n+1)} \Psi^{L-n+1)}}_{n-1\text{ iterated integrals}} \\ 
    &\int_{E_{L-n}} y^{L-n} j^{a}_{L-n}j^{b}_{L-n+1}\; dj_{L-n}\dots dj_L
  \end{aligned}
  \end{equation}
  As aforementioned, proving the $n=1$ case is required because for $n=1$, \eqref{eq:gradNGen} has a section of $n-1 = 0$ iterated integrals which cannot be possible for the proceeding logic.

  We now use the order invariance properly of iterated integrals (that is, $\int_A\int_B f(x,y)\;dxdy = \int_B\int_A f(x,y)\;dydx$) and reverse the order of integration of \eqref{eq:gradNGen}.

  In order to reverse the order of integration we must ensure each iterated integral has an integrand which contains variables which are guaranteed integration over some region. To examine this, we propose the following recurrence relation for the gradient. 

  Let $\{B_s\}$ be defined along $L -n \leq s \leq L$, as follows
  \begin{equation}
  \begin{aligned}
    B_L &= \int_{E_{L}} \left[\scripto(\gamma) - \delta\right] 
      \Psi^{L} B_{L-1} \;dj_L, \\
    B_s &= \int_{E_{\ell}} \Psi^{\ell}
     \sum_a^{Z^{\ell}_X} \sum_b^{Z^{\ell}_Y} j_\ell^a j_{\ell}^b B_{\ell} \; dj_\ell, \\
    B_{L-n} &= \int_{E_{L-n}} j_{L-n}^x j_{L-n+1}^y \; dj_{L-n}
  \end{aligned}
  \end{equation}
  such that $\frac{\partial E}{\partial k_{x,y}^{\ell}} = B_L$. If we wish to reverse the order of integration, we must find a reoccurrence relation on a sequence,
  $\{\rotB_s\}$  such that $\frac{\partial E}{\partial k_{x,y}^{L-n}} = \rotB_{L-n} = B_L.$ Consider the gradual reversal of \eqref{eq:gradNGen}.

Just as important as
  Clearly,
  \begin{equation} \label{eq:rev1}
  \begin{aligned}
    \frac{\partial E}{\partial k_{x,y}^{\ell}} =
      \int_{E_{L-n}}&  y^{L-n} j^{x}_{L-n}
      \int_{E_{L}}[\scripto(\gamma)-\delta] \Psi^{L} 
      \int_{E_{L-1}} w^{L-1} \Psi^{L-1} \\ & 
      \idotsint_{E_{L-n+1)}} j^{y}_{L-n+1}w^{L-n+1)} \Psi^{L-n+1)}  \; dj_{L-n+1}\dots dj_L dj_{L-n}
  \end{aligned}
  \end{equation} 
  is the first order reversal of \eqref{eq:gradNGen}. We now show the second order case with first weight function expanded.
  \begin{equation}\label{eq:rev2}
  \begin{aligned}
    \frac{\partial E}{\partial k_{x,y}^{\ell}} =
      \int_{E_{L-n}}&  y^{L-n}  j^{x}_{L-n}
      \int_{E_{L-n+1)}} \sum_b^{Z_Y} \sum_a^{Z_X} k_{a,b} j_{L-n+1}^{a+y} \Psi^{L-n+1)}
      \int_{E_{L}}[\scripto(\gamma)-\delta] \Psi^{L} \\ & 
      \idotsint_{E_{L-n+1)}} j^b_{L-n+2} w^{(L-n+2)} \Psi^{(L-n+2)}  \; dj_{L-n+1}\dots dj_L dj_{L-n}.
  \end{aligned}
  \end{equation}

  Repeated iteration of the method seen in \eqref{eq:rev1} and \eqref{eq:rev2}, where the inner most integral is moved to the outside of the $(L-s)^\mathrm{th}$ iterated integral, with $s$ is the iteration, yields the following full reversal of \eqref{eq:gradNGen}. For notational simplicity recall that $l = L-n$, then
 \begin{equation}\label{eq:revn}
  \begin{aligned}
    \frac{\partial E}{\partial k_{x,y}^{\ell}} =&
      \int_{E_{\ell}}  y^{\ell}  j^{x}_{l}
      \int_{E_{\ell}} \sum_a^{Z^{\ell}_X} j_{\ell}^{a+y} \Psi^{\ell}
      \int_{E_{\ell+2}} \sum_b^{Z_Y^{\ell}} \sum_c^{Z_X^{\ell+2}}
         k^{\ell}_{a,b} j^{b+c}_{l+2} \Psi^{\ell+2} \\&
      \int_{E_{\ell+3}} \sum_d^{Z_Y^{\ell+2}} \sum_e^{Z_X^{\ell+3}}
         k^{\ell+2}_{c,d} j^{d+e}_{l+3} \Psi^{\ell+3} 
      \idotsint_{E_{L}} \sum_q^{Z^{L-1}_Y} k^{L-1}_{p,q} j_L^q 
       \; [\scripto(\gamma)-\delta] \Psi^{L} \\ &
      \qquad \qquad dj_{L}\dots dj_{L-n}.
  \end{aligned}
  \end{equation}

  Observing the reversal in \eqref{eq:revn}, we yield the following recurrence relation for $\{\rotB_s\}$. Bare in mind, $l= L-n$, $x$ and $y$ still correspond with $\frac{\partial E}{\partial k^{\ell}_{x,y}}$, and the following relation uses its definition on $s$ for cases not otherwise defined.
  \begin{equation} \label{eq:rotBrelation}
  \begin{aligned}
    \rotB_{L,t} &= \int_{E_{L}}  \sum_b^{Z^{L-1}_Y} k^{L-1}_{t,b} j_L^b 
      \left[\scripto(\gamma) - \delta\right] \Psi^{L}\;dj_L. \\
    \rotB_{s,t} &= \int_{E_{(s)}}\sum_b^{Z^{(s-1)}_Y} \sum_a^{Z^{(s)}_X} 
      k^{(s-1)}_{t,b} j_s^{a+b} \Psi^{(s)} \rotB_{s+1,a}\; dj_s. \\
    \rotB_{\ell} &= \int_{E_{\ell}} \sum_a^{Z^{\ell}_X}
      j^{a+y}_{\ell} \Psi^{\ell} \rotB_{l+2, a}\; dj_{\ell}. \\
     \frac{\partial E}{\partial k^{\ell}_{x,y}} = \rotB_{l} &= \int_{E_{\ell}}
      j_{l}^x y^{\ell} \rotB_{\ell}\; dj_\ell.
  \end{aligned}
  \end{equation}
  Note that $\rotB_{L-n} = B_L$ by this logic.

  With \eqref{eq:rotBrelation}, we need only show that $\rotB_{L-n}$ is integrable. Hence we induct on $L-n \leq s \leq L$ over $\{\rotB_s\}$ under the proposition that $\rotB_s$ is not only numerically integrable but also constant. 

  Consider the base case $s = L$. For every $t$,
  because every function in the integrand of $\rotB_L$ in \eqref{eq:rotBrelation} is composed of $j_L$, functions of the form $\rotB_L$ must be numerically integrable and clearly, $\rotB_L \in \mathbb{R}$.

  Now suppose that $\rotB_{s+1,t}$ is numerically integrable and constant. Then, trivially, $\rotB_{s,u}$ is also numerically integrable by the contents of the integrand in \eqref{eq:rotBrelation} and $\rotB_{s,u} \in \mathbb{R}$. Hence, the proposition that $s+1$ implies $s$ holds for $\ell < s < L$.

  Lastly we must show that both $\rotB_{\ell}$ and $\rotB_{l}$ are numerically integrable. By induction $\rotB_{l+2}$ must be numerically integrable. Hence by the contents of its integrand $\rotB_{\ell}$ must also be numerically integrable and real. As a result, $\rotB_l =  \frac{\partial E}{\partial k^{\ell}_{x,y}}$ is real and numerically integrable.

  Since we have shown that $ \frac{\partial E}{\partial k^{\ell}_{x,y}}$ is numerically integrable, $\nabla E$ must therefore be numerically evaluable as aforementioned. This completes the proof.
\end{proof}
\begin{algorithm}[tb]
   \caption{Error Backpropagation}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} input $\gamma$, desired $\delta,$ learning rate $\alpha,$ time $t.$
   \FOR{$\ell \in \{0, \dots, L\}$}
    \STATE Calculate $\Psi^{\ell}=g'\left(\int_{E_{(\ell -1)}}{y^{(\ell -1)} w^{(\ell -1)}\ dj_{\ell}}\right)$
   \ENDFOR
   \STATE For every $t$, compute  $\rotB_{L,t}$ from from \eqref{eq:rotBrelation}.
   \STATE Update the output coefficient matrix
          $k_{x,y}^{L-1} - I_x^{L-1}
                  \int_{E_{L}} \left[\mathcal{F}(\gamma) - \delta\right] 
                    \Psi^{L} j_L^y \; dj_L \to  k_{x,y}^{L-1}.$
    \FOR{$l = L-2$ \textbf{to} $0$}
    \STATE If it is null, compute and memoize $ \rotB_{l+2,t}$ from \eqref{eq:rotBrelation}.
    \STATE Compute but do not store $\rotB_{\ell} \in \mathbb{R}.$
    \STATE Compute $\frac{\partial E}{\partial k_{x,y}^{\ell}} = \rotB_l$ from from \eqref{eq:rotBrelation}.
    \STATE Update the weights on layer $l$: $k_{x,y}^{\ell}(t) \to k_{x,y}^{\ell} $
    \ENDFOR
\end{algorithmic}
\end{algorithm}


With the completion of the implementation, the theoretical exposition of operator neural networks is complete.



\section{Conclusion}
In this paper we first extended the standard ANN recurrence relation to infinite dimensional input and output spaces. In this context of this new algorithm, ONNs, we proved two new universal approximation theorems. The proposition of operator neural networks lead to new insights into the black box model of traditional neural networks.

 Operator neural networks networks are a logical generalization of the discrete neural network and therefore all theorems shown for traditional neural networks apply to piecewise operator neural networks. Furthermore the creation of homologous theorems for universal approximation provided a way to find a relationship between the weights of traditional neural networks. This suggests that the discrete weights of a normal artificial neural network can be transformed into continuous surfaces which approximate kernels satisfying the training dataset. We then showed that operator neural networks are also able to approximate bounded linear operators.

The desire to implement $\scripto$ in actual learning problems motivated the exploration of a new space of algorithms, DFMs. This new space not only contains standard ANNs and ONNss but also similar extensions such as that proposed in \cite{roux}. We then showed that a subset of DFMs containg algorithms called continuous classifiers actually reduce the dimensionality of the input data when expressed in $\mathfrak{f}$ instead of $\mathfrak{n}$ layers. 

Finally  we proposed computationally feasible error backpropagation and forward propagation algorithms (up to an approximation).


\subsection{Future Work}
Although we have shown that advantage of using different subset of DFMs for learning tasks, there is still much work to be done. In this paper we did not explore different classes of weight surfaces, some of which may provide better computational integrability. It was also suggested to us that $\scripto$ may link kernel learning methods and deep learning. Lastly, it remains to be seen how the general class of DFMs, especially continuous classifiers, can be applied in practice.

==> sections/input_invariance.tex <==
%!TEX root = ../main.tex
\section{Input Invariance and Expressivity}

The main question of this work is how expressive are certain $\scriptf$ versus normal $\scriptn$ when assumptions are made on the type and graph topology of input functions. With respect to the original problem, it is natural to wonder if there are parameterizations for $\scriptf$ which avoid a cardinal dependence on the resoltuion of the input data. A basic such parameterization of $\scriptf$ are polynomial weight functions on every $\mathfrak{o}$ and $\mathfrak{f}$ layer.

That is for some functional neuyral network, we have that $\omega_\ell$ is parameterized by a polynomial, and
    \begin{equation}
\omega_\ell(u,v) = 
    \sum_{b}^{Z^{(l)}_Y} \sum_{a}^{Z^{\ell}_X} k^{\ell}_{a,b}u^{a}v^{b}.
\end{equation}
where $Z^\ell_X$ is the a polynomial order parameter.
In construction every single weight polynomial can capture lower-order properties of the weight surface with even less
dimensionality than a typical piecewise weight surface ($W_ij$). In fact polynomials can best-fit a function of $n$ discrete points in the worst case with $n$ coefficients, but they typically perform better within some $\epsilon$ error.
[ Numerical Methods of Curve Fitting. By P. G. Guest, Philip George Guest. Page 349.]
The key here is that the resolution of the input function $\xi$ only affects the feed-forward step
on the first $\mathfrak{f}$ layer, and not the number, $n$, of parameters $k_{a,b}$ in the model.


Suppose in some instance we have a weight polynomial on an $\mathfrak{f}$ with $M \in O(1)$ parameters, which has learned a model. Then the following theorem gives a direct comparison of an ANN performing the same task.

\begin{theorem}
  Let $\mathcal{F}$ be a functional neural network with only one $\mathfrak{f}$ functional layer. If a continuous function, say $f(t)$ is sampled uniformly from $t = 0$, to $t = N$, such that $x_n = f(n)$, and if $\mathcal{F}$ has an input function which is piecewise linear with

  \begin{equation}
  \xi = \left(x_{n+1} - x_n\right)\left(z - n\right) + x_n
  \end{equation}

  for $n \leq z < n+1$, then there exist some discrete neural network $\mathcal{N}$ such that $\mathcal{F}(\xi) = \mathcal{N}(\pmb{x}).$
\end{theorem}
\begin{proof}
  Recall that for the $j$th output neuron of a single layer discretized neural network,
  \begin{equation}
    \mathcal{N}_j(\pmb{x}) = g\left(\sum^N_{i=1}w_{i,j}x_i + \beta\right).
  \end{equation}
  Let this $\mathcal{N}$ compose the same sigmoid as the aforementioned $\mathfrak{f}$ functional layer. We need only show that equivalence holds on the inside.


  Because the definition of a network at the $j$th componet gives us

  \begin{equation}  \label{eq:n2nrelation}
    \mathcal{F}_j(\xi) = g\left(\mathfrak{f}[\xi] + \beta\right),
  \end{equation}
  it follows that,
  \begin{equation} \label{eq:n2piecewisein}
  \begin{aligned}
    \mathfrak{f}(\xi) &= \int_R\xi(t)\;\omega_j(t)\;dt \\ 
     &= \sum_n^{N-1}\int_n^{n+1} \left((x_{n+1} - x_n)(z - n) + x_n\right) \omega_j(z)\;dz\\ 
      &= \sum_n^{N-1}(x_{n+1} - x_n) \\
      &\hspace*{1cm}\times \int_n^{n+1} (z - n) \sum_m^M k_{m,j} z^m\;dz\\
      &\hspace*{1cm} + x_n\int_n^{n+1} \omega_j(z)\;dz\\
        &= \sum_n^{N-1}(x_{n+1} - x_n)\\
        &\hspace*{1cm} \times \sum_m^M k_{m,j} \left[\frac{1}{m+2}z^{m+2} - \frac{nz^{m+1}}{m+1}\right]_n^{n+1}\\
        &\hspace*{1cm}  + \sum_m^M k_{m,j} x_n \frac1{m+1}z^{m+1}\Big|^{n+1}_n
      \end{aligned}
      \end{equation}
      \\
      Now, let $V_{n,j} = \sum_m k_{m,j} \left[\frac{1}{m+2}z^{m+2} - \frac{nz^{m+1}}{m+1}\right]_n^{n+1}$ and $Q_{n,j} = \sum_m k_{m,j} \frac1{m+1}z^{m+1}\big|^{n+1}_n.$ We can now easily simplify \eqref{eq:n2piecewisein} using the telescoping trick of summation.
      \begin{equation}
        \begin{aligned}
        \mathfrak{f}(\xi) &= x_NV_{N-1,j} \\
        &\hspace*{1cm}+ \sum_{n=2}^{N-1}x_n\left(Q_{n,j} - V_{n,j} + V_{n-1,j}\right)\\
        &\hspace*{1cm} + x_1\left(Q_{1,j} - V{1,j}\right).
        \end{aligned}
      \end{equation}
      By simply letting $w_{1,j} = \left(Q_{1,j} - V_{1,j}\right), w_{n,j} = \left(Q_{n,j} - V_{n,j} + V_{n-1,j}\right),$ and $w_{N,j} = V_{N-1,j}$
      the following relation is satisfied,
      $\mathfrak{f}(\xi) = \mathfrak{n}(\pmb{x}).$
      Hence, $\mathcal{F}(\xi) = \mathcal{N}(\pmb{x})$ and the proof is complete.
    \end{proof}

    Notice that in the last proof, we went from $M \in O(1)$ dimensions to $O(N)$ 
    where $N$ is the number of samples on the input signal $\xi$! So there is constant space dimensionality
    reduction when using the $\mathfrak{f},$ and it is not to hard to see this for $\mathfrak{f}.$


